Fast hardware-aware matrix-free algorithm for higher-order finite-element discretized matrix multivector products on distributed systems

Recent hardware-aware matrix-free algorithms for higher-order finite-element (FE) discretized matrix-vector multiplications reduce floating point operations and data access costs compared to traditional sparse matrix approaches. This work proposes efficient matrix-free algorithms for evaluating FE discretized matrix-multivector products on both multi-node CPU and GPU architectures. We address a critical gap in existing matrix-free implementations, which are well suited only for the action of FE discretized matrices on a single vector. We employ batched evaluation strategies, with the batchsize tailored to underlying hardware architectures, leading to better data locality and enabling further parallelization. On CPUs, we utilize even-odd decomposition, SIMD vectorization, and overlapping computation and communication strategies. On GPUs, we employ strategies to overlap compute and data movement in conjunction with GPU shared memory, constant memory, and kernel fusion to reduce data accesses. Our implementation outperforms the baselines for Helmholtz operator action, achieving up to 1.4x improvement on one CPU node and up to 2.8x on one GPU node, while reaching up to 4.4x and 1.5x improvement on multiple nodes for CPUs ($\sim 3000$ cores) and GPUs ($\sim$ 25 GPUs), respectively. We further benchmark the performance of the proposed implementation for solving a model eigenvalue problem for 1024 smallest eigenvalue-eigenvector pairs by employing the Chebyshev Filtered Subspace Iteration method, achieving up to 1.5x improvement on one CPU node and up to 2.2x on one GPU node while reaching up to 3.0x and 1.4x improvement on multinode CPUs ($\sim 3000$ cores) and GPUs ($\sim$ 25 GPUs), respectively.

==> commentedParts.tex <==
%% \linenumbers
% MATRIX MULTIPLICATION WAY


% Finite element (FE) methods are widely used in science and engineering to solve problems of practical interests; among which FE discretization in quantum mechanics problem has gained lots of momentum in the last two decades. Open source FE based implementation of Density Functional Theory (DFT) \cite{MOTAMARRI2020106853, DAS2022108473} is one such growing field where the FE discretization evident a real-space method to solve highly non-linear problems. In contrast to conventional methods of solving DFT, a systematic convergence is obtained for any materials system using FE basis discretization \cite{Dislocation}. Further, wide range of boundary conditions e.g., periodic, non-periodic and semi-periodic is implemented in this technique which is a bottleneck in other discretization methods e.g., Finite differences \cite{MOTAMARRI2020106853}. Moreover, the locality of the FE basis function makes it a suitable candidate for parallel scalability benefitting in large-scale all-electrons calculations. 

% Large-scale DFT calculations are utilized in plethora of applications e.g., all-electron calculations for modelling of dislocation cores \cite{PRLDis} in conductors and semi-conductors, charge transport in DNA molecules \cite{DNABack}, ion diffusivity and migration barrier predictions \cite{SolidSolid1,SolidSolid2}, spin-spin interactions in solid defects \cite{SpinSpin1,SpinSpin2}, etc. The variety of DFT applications demand a foundational bottleneck, i.e., the scalability of an 'efficient' parallel FE based method to improve the \emph{ab initio} calculation of tens of thousands electrons and thus, provides the motivation of the present study. 

% In the FE framework, the problem is posed into a FE discretized space in such a way that a FE discretized operator is formed which is either used to obtain its action on the FE discretized space or solving the FE discretized space for the given action of the operator. In both the cases, iterative solvers like Conjugate Gradients are usually implemented. The operator is posed as a sparse matrix and the space is posed as a vector in these cases. The action is computed as the matrix-vector product which is the central and the most time-consuming step in FE based methods. Such products are usually implmented either by sparse matrix-vector product kernels or by using linear algebra packages like PETSc or Trilinos. However, such methods are disadvantageous to utilize in DFT problems where the discretized FE space is posed as a \emph{multivector} consisting of tens of thousands of vectors for all-electron space. On the contrary, it is found that such computations can be efficiently obtained on multi-threaded architectures using dense matrix-multivector products with an extraction and assembly steps which reduces the memory footprints drastically \cite{DAS2022108473, DasGordon}. Modern hardware-aware architectures and algorithms for the evaluation of such products suggest that the memory bandwidth can be increasingly reduced to shift towards compute-bound evaluation by performing \emph{on-the-fly} evaluation of matrix-vector products without storing FE based cell level matrix information \cite{MF0,MF1}. Thanks to the tensor-structured nature of the FE basis functions, such algorithms benefit in imposing a universal approach to compute sequential tensor contraction for the FE space irrespective of the FE mesh size, orientation and information. Such on-the-fly approach is commonly known as the 'matrix-free' approach. 

% Even though the matrix-free approach has been extensively utilized as well as improved in the past decade \cite{MF0, MF1, MF2, MF3, MF4}, it can not be directly extended to DFT problems because (i) the multivectors provide a new dimension of complexity as 10-1000 vectors are needed to be evaluated in a go, and (ii) the FE basis usually used are of FE order at least equal to 6 which poses memory-bandwidth limitation when computing its action on a multivector. Sparse amount of works have been done in the past to surpass these bottlenecks \cite{Davydov2020} but no widely available implementation is present on the long standing problem. 

% This work proposes \emph{\textbf{@Gourab and Nikhil, please write the benefits you obtained from our work and structure of the paper. These two paragraphs include your novelty in our results.}}

%Finite element methods are widely used in science and engineering to solve problems of practical interest. In the finite-element (FE) framework, these problems usually involve the construction of a FE discretized operator and often require either computing their action on an FE discretized fields or solving (usually utilizing iterative solvers) for the FE discretized fields given the action of the operator on them. In both these cases evaluating the product of the sparse matrix (FE discretized operator) and the vector (FE discretized field) product is the computationally dominant step. Traditionally, these matrix-vector products are computed directly by sparse-matrix vector multiplication modules, this method will be referred to as the Global Sparse Matrix (GSM) method. In prior works\cite{Carey1988Element-by-elementComputations}, it has been shown that the evaluation of the action of the linear operator can be done efficiently on multi-core architectures using cell-level dense matrix-vector multiplications followed by the assembly of cell-level product vectors, this method will be referred to as the Local Dense Matrix (LDM) method. The LDM strategy has been employed for evaluating matrix-multivector products at the cell-level on both CPU only and hybrid CPU-GPU architectures, demonstrating good throughput performance. Recent hardware-aware algorithms for evaluating such matrix-vector multiplications suggest that on-the-fly matrix-vector products without storing the cell-level matrices reduce both arithmetic complexity and memory footprint\cite{Ljungkvist2017Matrix-FreeMeshes}\cite{Kronbichler2012AApplication}\cite{Davydov2020AMultigrid}. These algorithms exploit the tensor-structured nature of the finite-element basis functions and recast the 3D integrals involved in the matrix-vector products as a sequence of tensor contractions.

%This work proposes an efficient implementation procedure for the matrix-free algorithm to compute such matrix-multivector products on hybrid CPU-GPU architectures. We employ efficient vendor BLAS routines on CPUs to perform the underlying tensor contractions. On GPUs, the proposed implementation utilizes the concept of kernel fusion to minimize data access and efficiently utilizes the GPU shared memory and registers to pipeline data access and computation. Further, we also present a data layout for storing the FE discretized global multivector to minimize the non-contiguous data accesses during the extraction of the cell-level vector from the global vector resulting in efficient parallelization. 


%Consider the differential operator $\mathcal{F}:H^2(\Omega)\rightarrow H^1(\Omega)$, where $\Omega\subset\mathbb{R}^3$ such that $\mathcal{F}=\mu\nabla^2+\kappa(\bx)$, where $\mu\in \mathbb{R}$ and $\kappa(\bx):\Omega \rightarrow \mathbb{R}$ are the system parameters.


% We now proceed to discuss the test problems that will be used to benchmark our implementation.
% \subsection{Test Problems}
% The proposed implementation will be benchmarked on 2 representative problems.
% \begin{itemize}
%     \item \emph{Helmholtz equation:}
%     Choosing the  RHS to be $f^i$ and setting $\mu=\frac{1}{4\pi}$ and $\kappa=1$, and assuming homogenous Dirichlet boundary conditions in the reference problem reduces it to the Helmholtz problem.

%     Find $\bU$ such that
%     \begin{align}
%         \bK\bU+\bM\bU=\bF
%     \end{align}
%     This problem will be solved using the preconditioned CG method assuming $n_q=p$.
%     \item \emph{Kohn-Sham Eigenproblem:}
%     Choosing the  RHS to be $\lambda_i u^i$ and setting $\mu=\frac{1}{2}$ and letting $\kappa(\bx)$ be a smooth function, and assuming homogenous Dirichlet boundary conditions in the reference problem reduces it to the Kohn-Sham eigenproblem.

%     Find $\Lambda$ and $\bU$ such that
%     \begin{align}
%         \bK\bU+\bM^\kappa\bU=\bM\bU\Lambda
%     \end{align}
%     This problem will be solved using the Chebyshev Filtered Subspace Iteration (ChFSI) algorithm assuming $n_q=p+2$.
% \end{itemize}
% Introduction to Global Sparse Matrix and Local Dense Matrix products for Multivector
% Consider a generic Finite Element (FE) discretized linear operator, represented by a global sparse matrix, $\bm{A}$, of size $N_{dofs}\times N_{dofs}$ and an input multivector, represented by a matrix $\bm{X}$ of $N_{dofs}$ rows and $N_v$ columns, where $N_{dofs}$ is the number of degrees of freedom, and $N_v$ is the number of vectors in the multivector. The action of the linear operator can then be represented by a sparse-matrix dense-matrix multiplication, i.e., $\bm{Y} = \bm{A}\bm{X}$, where the $n^{th}$ column of $\bm{Y}$ is the output vector corresponding to the $n^{th}$ input vector. 

% \subsection{Local Dense Matrix (LDM) approach}
% The LDM method for evaluating the action of the linear operator can be described in the following 3 steps: 
% \begin{enumerate}
%     \item \emph{Extraction}: Extract cell-level multivectors $\bm{U^e}$ as $N_{cells}$ matrices of $p^3$ rows and $N_v$ columns from $\bm{X}$, i.e., $\bm{U^e}\xleftarrow[]{}\bm{X}$
%     \item \emph{Multiplication}: Build cell-level dense matrices $\bm{H^e}$ of size $p^3\times p^3$ and evaluate the cell level output vectors, $\bm{V^e} = \bm{H^e}\bm{U^e}$.
%     \item \emph{Assembly}: Finally, assemble back the cell-level output multivectors $\bm{V^e}$ to the global output multivector $\bm{Y}$, i.e., $\bm{Y}\xleftarrow[]{}\bm{V^e}$
% \end{enumerate}
% The multiplication step can be implemented by using the strided batched BLAS gemm modules available in modern math libraries like Intel\textsuperscript{\textregistered} \texttt{MKL} for CPUs and the \texttt{cuBLAS} library for GPUs.

% % Matrix Free Method introduction
% \subsection{Matrix free (MF) approach}
% % Definition and introduction
% The matrix-free method for multivector is introduced using two linear operator prototypes, i.e., (a) the mass matrix and (b) the stiffness matrix.

% The mass matrix and the stiffness matrix are defined as $M_{ij}=\int_{\Omega} \hat N_i\hat N_jd\tau$ and $K_{ij}=\int_{\Omega} \nabla\hat N_i\cdot \nabla\hat N_jd\tau$ where $\hat N_i$ are the FE basis functions and $\Omega$ is the domain. The cell level mass matrix and the cell level stiffness matrix are written as $M_{ij}^e=\int_{\Omega_e} \hat N_i\hat N_jd\tau=\int_{\Omega_{ref}}  N_i N_j\left|\det{J}\right|d\tau$ and  $K_{ij}^e=\int_{\Omega_e} \nabla\hat N_i\cdot \nabla\hat N_jd\tau=\int_{\Omega_{ref}}  \left(J^{-1}\nabla N_i\right)\cdot\left(J^{-1}  \nabla N_j\right)\left|\det{J}\right|d\tau$, where $ N_i$ are the FE basis functions on reference cell, $J$ is the Jacobian matrix for the transformation from FE domain cell to the reference cell and $\Omega_{ref}$ is the reference domain. The mass matrix and stiffness matrix multivector products in the cell $e$ can be evaluated as,
% \begin{gather}
%     \left(\bm{M^eU^e}\right)_{ik} = \sum_j M^e_{ij}U^e_{jk}=\sum_q \det(J(\xi_q)) w_q N_i(\xi_q)\sum_j N_j(\xi_q)U_{jk} \label{massMatrix}\\
%     \left(\bm{K^eU^e}\right)_{ik} = \sum_j K^e_{ij}U^e_{jk}=\sum_q \det(J(\xi_q)) w_q \left(\nabla N_i(\xi_q)\right)^T\left(J(\xi_q)\right)^{-T}\left(J(\xi_q)\right)^{-1}\sum_j \nabla N_j(\xi_q)U_{jk} \label{laplaceMatrix}
% \end{gather}
% where $\xi_q$ are the quadrature points and $w_q$ are the quadrature weights. 

% For the specific case of a tensor structured basis, often the casi in FE discretization, the concept of sum factorization allows us to reduce the arithmetic complexity and the memory footprint further.
% \subsection{Sum factorization}
% The shape function matrix $\bf N$ in 3D is generally constructed from tensor products of low-level 1D polynomials. In such cases, the sum factorization method can be levied for efficient evaluation of the LDM. Without loss of generality, we decompose the LDM, (i.e., strided matrix multiplication of $\bf {NU}$) in 3 steps: (a) Interpolation, (b) Jacobian point products, and (c) Integration. First, the interpolant $\bm{U}^h_k$ is evaluated by tensor contraction of 1D basis function $S_i(\xi_q^{1D})$ as,
% \begin{equation}
%     \bm{U}^h_k = \left[S_{i,z}(\xi_{q,z}^{1D}) \otimes S_{i,y}(\xi_{q,y}^{1D}) \otimes S_{i,x}(\xi_{q,x}^{1D}) \right] \bm{U}_k
%     \label{TF}
% \end{equation}
% Here, $x,y,z$ denotes the Cartesian coordinates for the FE mesh. Moreover, The $i^{th}$ index of multivector $\bm{U}_k$ can be written in the multidimensional form as $(\bm{U}_k)_{i_x, i_y, i_z}$, where $(i_x, i_y, i_z)$ denotes the coordinate of the $i^{th}$ node. Then eq. (\ref{TF}) can be recast into sequential tensor contractions given by,
% \begin{equation}
%     \bm{U}^h_k = \sum_{i_z}^p S_{i_z,q_z} \sum_{i_y}^p S_{i_y,q_y} \sum_{i_x}^p S_{i_x,q_x} (\bm{U}_k)_{i_x, i_y, i_z}
%     \label{SF}
% \end{equation}
% Eq. (\ref{SF}) elucidates that the contraction of $\bm{U}_{k_{i_x, i_y, i_z}}$ is implemented in $i_x, i_y$ and $i_z$ indices respectively. The geometrical interpretation of eq. (\ref{SF}) is evaluating the $x-, y-$ and $z-$direction shape functions independently. A simple pictorial description is represented (see figure (\ref{Fig1})) to elucidate the above method in a three-dimensional FE operation of degree 1. In such case, the $S_i$ matrix is of size $2 \times 2$ representing $2$ quadrature points in each direction as shown in figure \ref{Fig1}(a). The interpolation is then carried out in x-direction irrespective of the other two directions. In the next step, the evaluated $x$-interpolant is interpolated in $y-$ direction and finally in the $z-$ direction as shown in Fig. (\ref{Fig1}(b),(c),(d)). 
% \begin{figure}
%     \centering
%     \includegraphics[width = \textwidth]{Fig1.jpg}
%     \caption{Sum factorization for three-dimensional FE operation on a reference cell of polynomial degree 1 (a) Node numbering in the reference cell (b) tensor contraction in $x-$ direction (c) tensor contraction in $y-$ direction (d) tensor contraction in $z-$ direction}
%     \label{Fig1}
% \end{figure}
% The mass matrix i.e., eq. (\ref{massMatrix}) is evaluated using sum factorization as,
% \begin{equation}
%     (N_j,\bm{U}^h_k)_{\Omega_k} \approx \sum_{q_z}^pS_{j_z,q_z}\sum_{q_y}^pS_{j_y,q_y}\sum_{q_x}^pS_{j_x,q_x}w_q\left|{J}^k_q\right|\sum_{i_z}^p S_{i_z,q_z} \sum_{i_y}^p S_{i_y,q_y} \sum_{i_x}^p S_{i_x,q_x} (\bm{U}_k)_{i_x, i_y, i_z}
%     \label{SF_1}
% \end{equation}
% Here, the multi-indices of $i,j,q$ represent the coordinate number discussed above. Further, the brute implementation strategy for the sum factorization is represented in algorithm (\ref{AlgoMM}).
% \begin{algorithm}
% \caption{Mass matrix operator with sum factorization}
% \label{AlgoMM}
% \begin{enumerate}
%     \item Interpolation of multivector $\bm{U}_k$. (\ref{SF_1}).
%     \item Preparation of the integrand by quadrature weights and determinant of Jacobians, i.e, $\bm{T}_k^q = w_q \det{J_k(x_q)u^h_{n,k}}$
%     \item Local cell multivector integration on each quadrature point $q$, i.e., $\bm{V}_k = \sum_{q_z}^pS_{j_z,q_z}\sum_{q_y}^pS_{j_y,q_y}\sum_{q_x}^pS_{j_x,q_x} \bm{T}_k^q$  
% \end{enumerate}
% \end{algorithm}

% On the other hand, the Laplace operator includes derivatives in the 3-dimensions. Similar to the sum factorization for the mass matrix, the derivative of the interpolant in the $i^{th}$ direction of multi-index $(i_x, i_y, i_z)$ (i.e., $\partial u^h_{n,k}/ \partial x_i$) is given by,  
% \begin{equation}
%     \frac{\partial \bm{U}^h_k}{\partial x} = \sum_{i_z}^p S_{i_z,q_z} \sum_{i_y}^p S_{i_y,q_y} \sum_{i_x}^p D_{i_x,q_x} (\bm{U}_k)_{i_x, i_y, i_z}
%     \label{LL1}
% \end{equation}
% Where $D_{i_x,q_x}$ is the derivative of $S_{i_x,q_x}$ in the $x^{th}$ direction. Using equation (\ref{LL1}), the Laplace operator is then evaluated by sum factorization as discussed in algorithm (\ref{AlgoLL}).
% \begin{algorithm}
% \caption{Laplace operator with sum factorization}
% \label{AlgoLL}
% \begin{enumerate}
%     \item Local multivector derivative interpolation on each vector $n$ and in each cell $k$. 
%     \begin{equation}
%         \begin{pmatrix}
%            \partial_x \bm{U}^h_k \\
%            \partial_y \bm{U}^h_k \\
%            \partial_z \bm{U}^h_k
%         \end{pmatrix} = \begin{pmatrix}
%                         \sum_{i_z}^p S_{i_z,q_z} \sum_{i_y}^p S_{i_y,q_y} \sum_{i_x}^p D_{i_x,q_x} \\
%                         \sum_{i_z}^p S_{i_z,q_z} \sum_{i_y}^p D_{i_y,q_y} \sum_{i_x}^p S_{i_x,q_x}\\
%                         \sum_{i_z}^p D_{i_z,q_z} \sum_{i_y}^p S_{i_y,q_y} \sum_{i_x}^p S_{i_x,q_x}
%                         \end{pmatrix}(\bm{U}^h_k)_{(i_x,i_y,i_z)}
%     \end{equation}
%     \item Integrand preparation by quadrature weights and determinant of Jacobians as well as the conversion of reference cell to real cell evaluation by inverse Jacobians.  
%     \begin{equation*}
%         (\bm{T}_k)_{(q_x,q_y,q_z)} = \left(J_k^{-T}(\xi_q)w_q\det{J_k(\xi_q)}J_k^{-1}(\xi_q)\right)\begin{pmatrix}
%            \partial_x \bm{U}^h_k \\
%            \partial_y \bm{U}^h_k \\
%            \partial_z \bm{U}^h_k
%         \end{pmatrix}
%     \end{equation*}
%     \item Local cell multivector integration on each quadrature point $q$.
%     \begin{equation}
%          \partial_x(\bm{V}_k) = \sum_{i_z}^p S_{i_z,q_z} \sum_{i_y}^p S_{i_y,q_y} \sum_{i_x}^p D_{i_x,q_x} (\bm{T}_k)_{(q_x,q_y,q_z)} 
%     \end{equation}
%     \begin{equation}
%         (\bm{V}_k) = \partial_x(\bm{V}_k) + \partial_y(\bm{V}_k) + \partial_z(\bm{V}_k)
%     \end{equation}      
% \end{enumerate}

% \end{algorithm}



% \subsection{GPU implementation}
% \subsubsection{Extraction}
% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width = \textwidth]{Extraction_1.jpg}
%     \caption{Sum factorization for three-dimensional FE operation on a reference cell of polynomial degree 1 (a) Node numbering in the reference cell (b) tensor contraction in $x-$ direction (c) tensor contraction in $y-$ direction (d) tensor contraction in $z-$ direction}
%     \label{Fig2}
% \end{figure*}
% The first step in the cell-level linear operation is extracting the cell-level vector $\bf U$ from $\bf X$, as discussed in section 2. A pictorial representation of the operation is showcased in fig. (\ref{Fig2}). A multivector can be represented as $N_v$ vectors of the same mesh form as shown in fig. (\ref{Fig2}(a)). For simplicity 4 cells arranged lexicographically as $\left[k-1, k+2\right]$. These cells are highlighted as red, yellow, green, and blue, respectively. The concept of extraction is elucidated with 1 dof shared among the 4 cells. For the $n^{th}$ vector, the dof is then broadcasted to 4 cells as shown in fig. (\ref{Fig2}(c)). It is noted that the extracted $\bf U$ is decomposed into several chunks and distributed to different threadblocks (TBs) as shown in fig. (\ref{Fig2}(c)). It decreases the memory throughput as the shared memory local to each TB can be utilized to compute the matrix-matrix product in the next step. Further details of its implementation is shown in fig. (\ref{Fig3}) in 3 steps as follows: (i) $\bf X$ is the input vector which is copied from the host to the device's global memory as shown in fig. (\ref{Fig3}) with $N_v$ as the fastest index. (ii) In the next step, a redistributed multivector $\bf X^*$ is formed by distributing the dofs with $N_m$ ($< N_v$ := $N_v/N_m \in \mathbb{Z}$). The advantage of $\bf X^*$ is in 2 folds: (a) it leads to finer parallelization as the matrix-free operations are independent of vectors and can be implemented over $N_v/N_m$ batches, and (b) it uses redesigned map to reduce required memory transactions by better utilizing the GPU cache lines and reduces the unavoidable non-contiguity arising from maps that form $U$ with $N_v$ fastest index. (iii) Finally, the $X^*$ is broadcasted to cell-level multivector where each cell is associated to an independent TB. The size of each TB is then $N_m \times p^3$ with $N_m$ fastest index. This leads to a finer level of parallelization in the matrix-matrix multiplication as the arithmetic operations of each cell for mass and Laplacian is computed for $N_m$ vectors independent of other cells. The choice of $N_m$ is crucial for decreasing the memory footprint as well as increasing the parallelization in the streaming multiprocessor (SM). It is a trade off whether to maximise the shared memory to its limit (i.e. 48 kB) or to form smaller TBs to fit more TBs for the arithmetic evaluation in the SM. in this case, maximising the shared memory to its upper bound is a viable choice as the time-consuming step of matrix-matrix multiplication is to be done for $N_m$ vectors in parallel in the shared memory. Fitting more TBs in SM by reducing the $N_m$ is not effective as the number of TBs instantiated is too larger than the maximum TBs that can be fitted with $N_m = 1$.       

% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width = \textwidth]{ExtractionThreads_Final.png}
%     \caption{Sum factorization for three dimensional FE operation on a reference cell of polynomial degree 1 (a) Node numbering in the reference cell (b) tensor contraction in $x-$ direction (c) tensor contraction in $y-$ direction (d) tensor contraction in $z-$ direction}
%     \label{Fig3}
% \end{figure*}

% \subsubsection{Sum Factorization}
% The sum factorization method is elucidated in algorithm which describes the 1D tensor contractions in the 3 directions to evaluate the shape function matrix $\bf N$ (i.e., eq. (\ref{SF})). It can then be utilized to obtain the mass matrix and Laplacian solution of the extracted multivector as discussed in algorithm (\ref{AlgoMM}, \ref{AlgoLL}). For simplicity we describe the GPU implementation of the interpolation step of degree 1 by following eq. (\ref{SF}) and fig. \ref{Fig1} and then we generalize the methodology for the evaluation of mass matrix and Laplacian operator for the multivectors extracted as described in the section 2.1. As the $S_{2 \times 2}$ matrix is utilized first to evaluate the tensor contraction of the quadratures in the x-direction, the evaluation is carried out a column major linear combination of the S matrix which is already loaded in the SM. In each TB, the multivector chunk can be written $U_{2\times 4 \times N_m}$ with $N_m$ as the fastest index. It is to be noted that the column-major linear combination of the row-major extracted multivector U eventually stores the data with a stride equal to p (i.e., 2) with $N_m$ as the fastest index. It is thus advantageous as it prevents $p^2$ (i.e., 4) bank conflicts to address the matrix-multivector multiplication in the y-direction. Similarly, the evaluation of tensor contraction in the y-direction eventually set up the multivector with a stride $p$ (i.e., 2) for the z-direction. Out of several methods and layouts, the discussed methodology is pragmatic and beneficial in several folds. First, it prevents the unavoidable bank conflicts due to the reshaping of the multivector for tensor contraction in each direction. Second, the use of the same matrix S across all multivectors irrespective of the TB increases the reusability of subsequent tensor contractions. Third, since it is already loaded to the SM, the evaluation of the linear combination can start as soon as the extraction of the data from the X is read without waiting for the whole data in the tensor contraction. This is advantageous as the tensor contractions use data access to its full compute potential and prevents re-reading the same data. Furthermore, the registers are kept to compute local as much as possible to each thread which reduces memory footprints even at the SM and thus, better utilizes the hardware. 

% In case of mass matrix evaluation for a 3D mesh, 6 such matrix multivector multiplication is performed, The first 3 evaluation is carried out to obtain the interpolation as discussed above. It is to be noted that the sum factorization in the z-direction results in the new multivector in the x-direction. Then point multiplication of the Jacobian and the quadrature points is implemented and finally another 3 sum factorization is implemented for integration step. The methological development of the linear combination of column-major multivector is advantageous in the integration step as the final output after the interpolation step is in the x-direction which is the fastest index for lexicographic numbering of each vector. 

% In case of Laplacian evaluation for a 3D mesh, 18 such matrix multivector multiplication is performed. Unlike mass matrix, in this case another matrix $D$ is loaded to the SM to evaluation the gradient in the sprecific direction as discussed in section 2. It is further noted that for the gradient evaluation in the y- and z-direction, the first matrix multivector multiplication in the x-direction is same. Thus, 1 such evaluation can be by-passed and the total number of matrix multivector evaluation is 17. 




% \subsection{Mass matrix}
% Discuss the methodology with a pictorial description on blocks and threads.
% \subsection{Laplace operator}
% Similarly we do for the Laplace operator.

% \subsection{Sum factorization implementation on CPUs}
% \subsubsection{Mass matrix}
% Discuss the methodology with a pictorial description of the CPU implementation in terms of blocks and threads for mass matrix.
% \subsubsection{Laplace operator}
% Similarly we do for the Laplace operator.

% \subsection{Extension to multivector FE solver}
% Only differentiate what to modify in the single vector approach. 

Considering a finite-dimensional test function space ${X}_p(\Omega)\subset \mathcal{V}$, the Galerkin form of the above problem seeks to find $u^i\in {X}_p(\Omega)\;\; \forall i=0,1,\dots,n-1$ such that 
\begin{equation}
    \begin{alignedat}{3}
    a(v,u^i)+(v,u^i)_\kappa&=\begin{cases}(v,f^i)\\\lambda_i(v,u^i)\end{cases} \qquad& &\forall v\in {X}_p\\
    u^i(\bx)&=\Pi u_D(\bx) & &\forall \bx \in \partial \Omega_D
    \end{alignedat}\label{eqn:galerkin}
\end{equation}
where $\Pi u_D$ is the interpolant of $u_D$ in ${X}_p(\Omega)$ and the bilinear forms are defined as 
\begin{align*}
    a(v,u^i)&=\int_{\Omega}\mu \nabla v\cdot\nabla u^i d\bx & (v,u^i)_\kappa&=\int_{\Omega}v\kappa u^i d\bx\\
    (v,u^i)&=\int_{\Omega}vu^id\bx & (v,f^i)&=\int_{\Omega}vf^id\bx 
\end{align*}

Expanding $u^i$ and $v$ in the basis of nodal Lagrange interpolating polynomials as $u^i(\bx)=\sum_{j=0}^{m-1} u_j^i\phi_j(\bx)$ and $v(\bx)=\sum_{j=0}^{m-1} v_j\phi_j(\bx)$ where $\phi_j(\bx)$ is the Lagrange interpolating polynomial defined at node $\bx_j$ and $m$ is the number of nodes, we define the vectors $\bu^i$ and $\bv$. We can then rewrite the bilinear forms as inner products
\begin{align*}
    a(v,u^i)&=\bv^T\bK \bu^i &(v,u^i)_\kappa&=\bv^T\bM^\kappa \bu^i\\
    (v,u^i)&=\bv^T\bM \bu^i& (v,f^i)&=\bv^T\bff^i 
\end{align*}
Here $\bK$ is the \emph{Stiffness Matrix} defined as $K_{ij}=a\left(\phi_i,\phi_j\right)$, $\bM^\kappa$ is the \emph{Weighted Mass Matrix} defined as $M^\kappa_{ij}=\left(\phi_i,\phi_j\right)_\kappa$, $\bM$ is the \emph{Mass Matrix} defined as $M_{ij}=\left(\phi_i,\phi_j\right)$ and $\bff^i$ is the \emph{force vector} defined as $f^i_j=\left(\phi_j,f^i\right)$.

Equation \ref{eqn:galerkin} is then reduced to finding $\bu^i\in \mathbb{R}^m\;\; \forall i=0,1,\dots,n-1$ such that
\begin{equation}
    \begin{alignedat}{3}
        \bK\bu^i&+\bM^\kappa \bu^i=\begin{cases}\bff^i\\\lambda_i\bM\bu^i\end{cases}\\
        u^i_j&=\Pi u_D(\bx_j) & &\forall \bx_j \in \partial \Omega_D
    \end{alignedat}\label{eqn:matrix}
\end{equation}

In order to solve equation \ref{eqn:matrixmultivector} via the Preconditioned Conjugate Gradient (PCG) method (in case the RHS is $\bF$) or via the Chebyshev Filtered Subspace iteration (ChFSI) method (in case the RHS is $\bM\bU\mathbf{\Lambda}$) efficient evaluation of the matrix multivector products $\bK\bU$, $\bM^\kappa \bU$ and $\bM\bU$ is paramount.


\begin{align}
    u^{i,h\,(e)}(\bx(\bxi))=&\sum_{J=1}^{n_p^3}u^{i,h,\,(e)}\left(\bx^{(e)}_{J}\right)\hat{N}_J\left(\bxi\right) \nonumber \\
    =&\sum_{j_1=1}^{n_p}\sum_{j_2=1}^{n_p}\sum_{j_3=1}^{n_p}u^{i,h,\,(e)}\left(\bx^{(e)}_{j_1,j_2,j_3}\right)\hat{N}^{1D}_{j_1}(\xi^0)\hat N^{1D}_{j_2}( \xi^1)\hat{N}^{1D}_{j_2}(\xi^3) \label{eqn:fecellvector}
\end{align}
where this Eq.~\eqref{eqn:fecellvector} exploits the tensor structured nature of the FE cell-level 3D Lagrange interpolating polynomials $\hat{N}_J()\bxi$ to 

while $\bx^e_{j_1j_2j_3}$ is the \cred cartesian \cn coordinate of the node indexed by $j_1,j_2,j_3$ in $\Omega^e$.

Consequently, we split the element index $e$ into a multi-index $e,t$. Imposing the continuity condition across subdomains, $\bx^{e_{1},t_1}_{j_1j_2j_3}=\bx^{e_{2},t_2}_{k_1k_2k_3}\implies u^{i,e_{1},t_1}\left(\bx^{e_{1},t_1}_{j_1j_2j_3}\right)=u^{i,e_{2},t_2}\left(\bx^{e_{2},t_2}_{k_1k_2k_3}\right)$ is done by defining a boolean sparse matrix termed the \emph{partitioner} matrix, $\bP^t$, which acts on $\bU$ to give the subdomain level multivector $\bU^t$.

Similarly, the continuity condition across elements within a subdomain, $\bx^{e_1,t}_{j_1j_2j_3}=\bx^{e_2,t}_{k_1k_2k_3}\implies u^{i,e_1,t}\left(\bx^{e_1,t}_{j_1j_2j_3}\right)=u^{i,e_2,t}\left(\bx^{e_2,t}_{k_1k_2k_3}\right)$ is done by the standard finite element processes of extraction and assembly. These processes can be done via a \emph{global to local map}, which can be mathematically represented as a sparse matrix multivector multiplication. In case of non-conforming meshes arising from adaptive mesh refinement, it is necessary to constrain the values of $\bU$ at certain nodes in order to ensure that $X_p^3(\Omega) \subset H^1(\Omega)$, this can be accomplished by using a constraint matrix $\bC$. The \emph{element-level multivector}, $U^{e,t}_{ij}=u^{i,e,t}_j$, can now be written as $\bU^{e,t}=\bQ^{e,t}\bC^t\bP^t\bU \;\forall e=1,2,\dots,E_t$ and $t=1,2,\dots,n_t$ where $\bU$ is the $m\times n_v$ matrix representing the \emph{global multivector}, $\bQ^{e,t}$ is an $n_p^3\times m_t$ boolean matrix representing the \emph{global to local map} on subdomain $t$ and $\bC^t$ is the $m_t\times m_t$ \emph{constraint matrix}.

Considering $\bA$ to be an FE discretized operator (such as $\bK$, $\bM^\kappa$ or $\bM$) we can now rewrite it in terms of the \emph{element-level operator matrix}, $\bA^e$, as
\begin{align}
    \bA = \sum_{t}^{n_t}{\bP^t}^T{\bC^t}^T\left(\sum_e^{E_t}{\bQ^{e,t}}^T\bA^e\bQ^{e,t}\right)\bC^t\bP^t\label{eqn:gsm}
\end{align} 
The evaluation of the $n_p^3\times n_p^3$ matrix $\bA^e$ can be efficiently done using the fact that all elements can be linearly mapped to $\hat\Omega$. For instance, the element-level stiffness matrix can be evaluated as
\begin{align}
    K^e_{ij}=\int_{\Omega^e}\mu \nabla  N_i\cdot\nabla  N_j d\bx=\int_{\hat\Omega}\mu \left(\left(\bJ^e\right)^{-T}\hat\nabla \hat N_i\right)\cdot\left(\left(\bJ^e\right)^{-T}\hat\nabla \hat N_j\right) \det{\bJ^e} d\hat\bx
\end{align}
where $\bJ^e$ is the Jacobian matrix of the map from $\Omega^e$ to $\hat\Omega$. Using a tensor structured $n_q$-point quadrature rule with quadrature points $\hat\bx_q$ and the quadrature weights $w_q$, the above integral can  be written as
\begin{align}
    K^e_{ij}=\sum_{q=1}^{n_q^3}\left(\hat\nabla \hat N_i\right)^T\left(\bJ^e\right)^{-1}\left(\bJ^e\right)^{-T}\left(\hat\nabla \hat N_j\right)\mu w_q\det{\bJ^e}\Biggl|_{\hat\bx_q}
\end{align}

\subsubsection{Evaluation via global sparse matrix}
The most straight-forward method is to evaluate the \emph{global operator matrix} as given by equation \ref{eqn:gsm} and evaluate the resulting sparse-matrix dense-matrix product.

\begin{alignedat}{1}
        \bV=\bA\bU&=\sum_{t}^{n_t}{\bP^t}^T{\bC^t}^T\left(\sum_e^{E_t}{\bQ^{e,t}}^T\bA^e\bQ^{e,t}\right)\bC^t\bP^t\bU\\&=\sum_{t}^{n_t}{\bP^t}^T{\bC^t}^T\left(\sum_e^{E_t}{\bQ^{e,t}}^T\bA^e\bU^{e,t}\right)\label{eqn:base}        
    \end{alignedat}
    
    A naive implementation of these equations, assuming that $\bN$ and $\bD^k$ matrices are precomputed, still has the computational complexity of $O(E(2n_q^3n_p^3+n_q^3)n_v)$ in case of mass matrix and $O(E(12n_q^3n_p^3+3n_q^3)n_v)$ in case of stiffness matrix when used in the \emph{FE-cell level evaluation} step.

% \begin{algorithm}[!ht]
%     \caption{Batchwise evaluation of ${\bV}$ on CPUs}\label{alg:vcpu}
%     \KwIn{${\bU}$}
%     \KwData{$\bB^{\left(i_b\right)},\bP^{\left(i_b,t\right)},\bC^{\left(i_b,t\right)},\bQ^{\left(i_b,e,t\right)},\bN^{1D},\bD^{1D},\bG,\bG^{sd}$ where $s,d=0,1,2$}
%     \KwTemp{$\bT, \bT^0,\bT^1,\bT^2$}
%     \KwResult{${\bV}$}

%     \KwTId{$t$}
%     $\bU^{t,1} \gets \bP^{t,1}\bB^{1}{\bU}$\;
%     \For{$i_b\gets1$ \KwTo $n_b$}{
%         \If{$i_b<n_b$}{Start : $\bU^{t,i_b+1} \gets \bP^{t,i_b+1}\bB^{i_b+1}{\bU}$\;}
%         \If{$i_b>1$}{Start : ${\bV} \gets \bV+{\bP^{t,i_b-1}}^T{\bB^{i_b-1}}^T{\bV}^{t,i_b-1}$\;}
%         $\bU^{\left(i_b,t\right)} \gets \bC^{\left(i_b,t\right)}\bU^{\left(i_b,t\right)}$\;
%         \For{$e\gets1$ \KwTo $E_t$}{
%             $\bT \gets \bQ^{\left(i_b,e,t\right)}\bU^{\left(i_b,t\right)}$\;
%             $\bT \gets \bN\bT$\;
%             $\bT^0 \gets \left(\bI\otimes\bI\otimes\bD^{1D}\otimes\bI\right)\bT$\;
%             $\bT^1 \gets \left(\bI\otimes\bD^{1D}\otimes\bI\otimes\bI\right)\bT$\;
%             $\bT^2 \gets \left(\bD^{1D}\otimes\bI\otimes\bI\otimes\bI\right)\bT$\;
%             $\bT_s \gets \displaystyle\sum_{d=0}^{2} \bG^{sd}\bT_d$\;
%             $\bT \gets \bG\bT$\;
%             $\bT \gets \bT+\left(\bI\otimes\bI\otimes\bD^{1D}\otimes\bI\right)^T\bT^0$\;
%             $\bT \gets \bT+\left(\bI\otimes\bD^{1D}\otimes\bI\otimes\bI\right)^T\bT^1$\;
%             $\bT \gets \bT+\left(\bD^{1D}\otimes\bI\otimes\bI\otimes\bI\right)^T\bT^2$\;
%             $\bT \gets \bN^T\bT$\;
%             $\bV^{\left(i_b,t\right)} \gets \bV^{\left(i_b\right)}+{\bQ^{\left(i_b,e,t\right)}}^T\bT$\;            
%                     }
%             $\bV^{\left(i_b,t\right)} \gets {\bC^{\left(i_b,t\right)}}^T\bV^{\left(i_b,t\right)}$\;
%             \If{$i_b<n_b$}{Finish : $\bU^{t,i_b+1} \gets \bP^{t,i_b+1}\bB^{i_b+1}{\bU}$\;}
%             \If{$i_b>1$}{Finish : ${\bV} \gets \bV+{\bP^{t,i_b-1}}^T{\bB^{i_b-1}}^T{\bV}^{t,i_b-1}$\;}
%                 }
%     ${\bV}^{t,n_b} \gets {\bP^{t,n_b}}^T{\bB^{n_b}}^T{\bV}^{t,n_b}$\;
%     \Return{${\bV}$}
% \end{algorithm}

% \begin{algorithm}[!ht]
%     \caption{Evaluation of ${\bV^{\left(i_b,t\right)}}$ on CPU architectures}\label{alg:vibtcpu}
%     \begin{algorithmic}
%         \Input ${\bU^{\left(i_b,t\right)}}$
%         \Require $\bC^{\left(i_b,t\right)},\bQ^{\left(i_b,e,t\right)},\bN^{1D},\bD^{1D},\bm{\kappa},\bJ^{\left(e\right)}$
%         \Temp $\bT, \bT^0,\bT^1,\bT^2$
%         \Result ${\bV^{\left(i_b,t\right)}}$

%         \MPIr $t$
%         \State $\bU^{\left(i_b,t\right)} \gets {\bC^{\left(i_b,t\right)}}\bU^{\left(i_b,t\right)}$
%         \For {$e:=1,\dots,E_t$}
%             \State $\bT \gets \bQ^{\left(i_b,e,t\right)}\bU^{\left(i_b,t\right)}$
%             \State $\bT \gets \bT{\bN^{1D}}^T$\Comment{equation \ref{eqn:tc3}}
%             \For {$q_3 := 1,\dots,n_q$}
%                 \State $\bT_{q_3} \gets \bT_{q_3}{\bN^{1D}}^T$\Comment{equation \ref{eqn:tc2}}
%             \EndFor
%             \For {$q_3 := 1,\dots,n_q$}
%                 \For {$q_2 := 1,\dots,n_q$}
%                     \State $\bT_{q_2,q_3} \gets \bT_{q_2,q_3}{\bN^{1D}}^T$\Comment{equation \ref{eqn:tc1}}
%                 \EndFor
%             \EndFor
%             $\bT^2 \gets \bT\mbox{${\tilde\bD}^{1D}$}^T$\Comment{equation \ref{eqn:tc3}}
%             \For {$q_3 := 1,\dots,n_q$}
%                 \State $\bT^1_{q_3} \gets \bT_{q_3}\mbox{${\tilde\bD}^{1D}$}^T$\Comment{equation \ref{eqn:tc2}}
%             \EndFor
%             \For {$q_3 := 1,\dots,n_q$}
%                 \For {$q_2 := 1,\dots,n_q$}
%                     \State $\bT^0_{q_2,q_3} \gets \bT_{q_2,q_3}\mbox{${\tilde\bD}^{1D}$}^T$\Comment{equation \ref{eqn:tc1}}
%                 \EndFor
%             \EndFor
%             \State $\left[\bT^0 \bT^1\bT^2\right] \gets \left[\bT^0 \bT^1\bT^2\right]{\bJ^{(e)}}^{-1}{\bJ^{(e)}}^{-T}\det{\bJ^{(e)}}\mu $
%             \State $\bT \gets \det{\bJ^{(e)}}\bm{\kappa}\circ \bT$
%             \State $\bT \gets \bT + \bT^2\mbox{${\tilde\bD}^{1D}$}$\Comment{equation \ref{eqn:tc3}}
%             \For {$q_3 := 1,\dots,n_q$}
%                 \State $\bT_{q_3} \gets \bT_{q_3}+ \bT^1_{q_3}\mbox{${\tilde\bD}^{1D}$}$\Comment{equation \ref{eqn:tc2}}
%             \EndFor
%             \For {$q_3 := 1,\dots,n_q$}
%                 \For {$q_2 := 1,\dots,n_q$}
%                     \State $\bT_{q_2,q_3} \gets \bT_{q_2,q_3}+ \bT^0_{q_2,q_3}\mbox{${\tilde\bD}^{1D}$}$\Comment{equation \ref{eqn:tc1}}
%                 \EndFor
%             \EndFor
%             \State  $\bT \gets \bT{\bN^{1D}}$\Comment{equation \ref{eqn:tc3}}
%             \For {$q_3 := 1,\dots,n_q$}
%                 \State $\bT_{p_3} \gets \bT_{p_3}{\bN^{1D}}$\Comment{equation \ref{eqn:tc2}}
%             \EndFor
%             \For {$q_3 := 1,\dots,n_q$}
%                 \For {$q_2 := 1,\dots,n_q$}
%                     \State $\bT_{p_2,p_3} \gets \bT_{p_2,p_3}{\bN^{1D}}$\Comment{equation \ref{eqn:tc1}}
%                 \EndFor
%             \EndFor
%             \State $\bV^{\left(i_b,t\right)} \gets \bV^{\left(i_b,t\right)}+{\bQ^{\left(i_b,e,t\right)}}^T\bT$
%         \EndFor
%         \State $\bV^{\left(i_b,t\right)} \gets {\bC^{\left(i_b,t\right)}}^T\bV^{\left(i_b,t\right)}$
%     \end{algorithmic}
%     \Return $\bV^{\left(i_b,t\right)}$
% \end{algorithm}

% \begin{algorithm}[!ht]
%     \caption{Evaluation of ${\bV^{\left(i_b,t\right)}}$ on CPU architectures}\label{alg:vibtcpu}
%     \begin{algorithmic}
%         \Input ${\bU^{\left(i_b,t\right)}}$
%         \Require $\bC^{\left(i_b,t\right)},\bQ^{\left(i_b,e,t\right)},\bN^{1D},\bD^{1D},\bm{\kappa},\bJ^{\left(e\right)}$
%         \Require \texttt{matmul}, see listing \ref{lst:cpusig}
%         \Temp $\bT_1, \bT_2$: arrays of size $3bn_q^3$
%         \Temp $\bT$: array of size $bn_q^3$
%         \Set  $\bT^0_1,\bT^1_1,\bT^2,_1$ arrays of size $bn_q^3$ such that $\bT_1=\left[\bT^0_1\; \bT^1_1\;\bT^2_1\right]$
%         \Set  $\bT^0_2,\bT^1_2,\bT^2,_2$ arrays of size $bn_q^3$ such that $\bT_2=\left[\bT^0_2\; \bT^1_2\;\bT^2_2\right]$
%         \Result ${\bV^{\left(i_b,t\right)}}$

%         \MPIr $t$
%         \State $\bU^{\left(i_b,t\right)} \gets {\bC^{\left(i_b,t\right)}}\bU^{\left(i_b,t\right)}$
%         \For {$e:=1,\dots,E_t$}
%             \State $\bT_1^0 \gets \bQ^{\left(i_b,e,t\right)}\bU^{\left(i_b,t\right)}$
%             \State matmul<$bn_p^2,n_q,n_p,1,0,1$\texttt{>}$\left(\bT_1^0,\bN^{1D},\bT_1^1\right)$\Comment{equation \ref{eqn:tc3}}
%             \State \texttt{matmul<}$bn_p,n_q,n_p,n_q,0,1$\texttt{>}$\left(\bT_1^1,\bN^{1D},\bT_1^0\right)$\Comment{equation \ref{eqn:tc2}}
%             \State \texttt{matmul<}$b,n_q,n_p,n_q^2,0,1$\texttt{>}$\left(\bT_1^0,\bN^{1D},\bT\right)$\Comment{equation \ref{eqn:tc1}}
%             \State \texttt{matmul<}$bn_q^2,n_q,n_q,1,0,1$\texttt{>}$\left(\bT,\tilde\bD^{1D},\bT_2^2\right)$\Comment{equation \ref{eqn:tc3}}
%             \State \texttt{matmul<}$bn_q,n_q,n_q,n_q,0,1$\texttt{>}$\left(\bT,\tilde\bD^{1D},\bT_2^1\right)$\Comment{equation \ref{eqn:tc2}}
%             \State \texttt{matmul<}$b,n_q,n_q,n_q^2,0,1$\texttt{>}$\left(\bT,\tilde\bD^{1D},\bT_2^0\right)$\Comment{equation \ref{eqn:tc1}}
%             \State \texttt{matmul<}$bn_q^3,3,3,1,0,1$\texttt{>}$\left(\bT_2,{\bJ^{(e)}}^{-1}{\bJ^{(e)}}^{-T}\det{\bJ^{(e)}}\mu,\bT_1\right)$
%             \State $\bT \gets \det{\bJ^{(e)}}\bm{\kappa}\circ \bT$

%             \State \texttt{matmul<}$bn_q^2,n_q,n_q,1,1,0$\texttt{>}$\left(\bT,_2^2\tilde\bD^{1D},\bT\right)$\Comment{equation \ref{eqn:tc3}}
%             \State \texttt{matmul<}$bn_q,n_q,n_q,n_q,1,0$\texttt{>}$\left(\bT_2^1,\tilde\bD^{1D},\bT\right)$\Comment{equation \ref{eqn:tc2}}
%             \State \texttt{matmul<}$b,n_q,n_q,n_q^2,1,0$\texttt{>}$\left(\bT_2^1,\tilde\bD^{1D},\bT\right)$\Comment{equation \ref{eqn:tc1}}

%             \State \texttt{matmul<}$bn_q^2,n_p,n_q,1,0,0$\texttt{>}$\left(\bT,\bN^{1D},\bT_1^0\right)$\Comment{equation \ref{eqn:tc3}}
%             \State \texttt{matmul<}$bn_q,n_p,n_q,n_p,0,0$\texttt{>}$\left(\bT_1^0,\bN^{1D},\bT\right)$\Comment{equation \ref{eqn:tc2}}
%             \State \texttt{matmul<}$b,n_p,n_q,n_p^2,0,0$\texttt{>}$\left(\bT,\bN^{1D},\bT_1^0\right)$\Comment{equation \ref{eqn:tc1}}


%             \State $\bV^{\left(i_b,t\right)} \gets \bV^{\left(i_b,t\right)}+{\bQ^{\left(i_b,e,t\right)}}^T\bT_1^0$
%         \EndFor
%         \State $\bV^{\left(i_b,t\right)} \gets {\bC^{\left(i_b,t\right)}}^T\bV^{\left(i_b,t\right)}$
%     \end{algorithmic}
%     \Return $\bV^{\left(i_b,t\right)}$
% \end{algorithm}

% \begin{algorithm}[!ht]
%     \caption{Evaluation of $\bV^{e,t}=\left(\bK^e+\bM^{\kappa,e}\right)\bU^{e,t}$}\label{alg:ve}
%     \begin{algorithmic}
%         \Input $\bU^{e,t}$
%         \Require $\bN^{1D},\tilde\bD^{1D},\bG,\bG^{sd}$ where $s,d=0,1,2$
%         \Temp $\bT, \bT_0,\bT_1,\bT_2$
%         \Result $\bV^{e,t}$
%         \State $\bT \gets \bN\bU^{e,t}$
%         \State $\bT_0 \gets \left(\bI\otimes\bI\otimes\tilde\bD^{1D}\otimes\bI\right)\bT$
%         \State $\bT_1 \gets \left(\bI\otimes\tilde\bD^{1D}\otimes\bI\otimes\bI\right)\bT$
%         \State $\bT_2 \gets \left(\tilde\bD^{1D}\otimes\bI\otimes\bI\otimes\bI\right)\bT$
%         \State $\bT_s \gets \displaystyle\sum_{d=0}^{2} \bG^{sd}\bT_d$
%         \State $\bT \gets \bG\bT$
%         \State $\bT \gets \bT+\left(\bI\otimes\bI\otimes\tilde\bD^{1D}\otimes\bI\right)^T\bT_0$
%         \State $\bT \gets \bT+\left(\bI\otimes\tilde\bD^{1D}\otimes\bI\otimes\bI\right)^T\bT_1$
%         \State $\bT \gets \bT+\left(\tilde\bD^{1D}\otimes\bI\otimes\bI\otimes\bI\right)^T\bT_2$
%         \State $\bV^{e,t} \gets \bN^T\bT$
%     \end{algorithmic}
%     \Return $\bV^{e,t}$
% \end{algorithm}
% \begin{algorithm}[!ht]
%     \caption{Evaluation of $\bT=\bN\bU^{e,t}$}\label{alg:NU}
%     \begin{algorithmic}
%         \Input $\bU^{e,t}$
%         \Require $\bN^{1D}$
%         \Result $\bT$
%         \State $\bT \gets \left(\bI\otimes\bI\otimes\bN^{1D}\otimes\bI\right)\bU^{e,t}$
%         \State $\bT \gets \left(\bI\otimes\bN^{1D}\otimes\bI\otimes\bI\right)\bT$
%         \State $\bT \gets \left(\bN^{1D}\otimes\bI\otimes\bI\otimes\bI\right)\bT$
%     \end{algorithmic}
%     \Return $\bT$
% \end{algorithm}
% \begin{algorithm}[!ht]
    %     \caption{Overlap of computation and communication}\label{alg:cpuoverlap}
    %     \begin{algorithmic}
    %         \Input ${\bU}$
    %         \Require $\bB^{\left(i_b\right)},\bP^{\left(i_b,t\right)},\bC^{\left(i_b,t\right)},\bQ^{\left(i_b,e,t\right)}$ for $e=1,\dots,E_t$ and $i_b=1,\dots,n_b$
    %         \Result ${\bV}$
    %         \MPIr $t$
    %         \State $\bU^{t,1} \gets \bP^{t,1}\bB^{1}{\bU}$
    %         \For{$i_b:=1,\dots,n_b$}
    %             \If{$i_b<n_b$}
    %                 \State Start : $\bU^{t,i_b+1} \gets \bP^{t,i_b+1}\bB^{i_b+1}{\bU}$
    %             \EndIf
    %             \If{$i_b>1$}
    %                 \State Start : ${\bV} \gets \bV+{\bP^{t,i_b-1}}^T{\bB^{i_b-1}}^T{\bV}^{t,i_b-1}$
    %             \EndIf
    %             \State $\bV^{\left(i_b,t\right)} \gets {\bC^{\left(i_b,t\right)}}^T\left(\sum_{e}^{E_t}{\bQ^{e,i_b,t}}^T\bA^{\left(e\right)}\bQ^{e,i_b,t}\right)\bC^{\left(i_b,t\right)}\bU^{\left(i_b,t\right)}$
    %             \If{$i_b<n_b$}
    %                 \State Finish : $\bU^{t,i_b+1} \gets \bP^{t,i_b+1}\bB^{i_b+1}{\bU}$
    %             \EndIf
    %             \If{$i_b>1$}
    %                 \State Finish : ${\bV} \gets \bV+{\bP^{t,i_b-1}}^T{\bB^{i_b-1}}^T{\bV}^{t,i_b-1}$
    %             \EndIf
    %         \EndFor
    %         \State ${\bV}^{t,n_b} \gets {\bP^{t,n_b}}^T{\bB^{n_b}}^T{\bV}^{t,n_b}$
    %     \end{algorithmic}
    %     \Return $\bV$
    % \end{algorithm}
    
